Wide-band Profile Domain Pulsar Timing Analysis

We extend profile domain pulsar timing to incorporate wide-band effects such as frequency-dependent profile evolution and broadband shape variation in the pulse profile. We also incorporate models for temporal variations in both pulse width and in the separation in phase of the main pulse and interpulse. We perform the analysis with both nested sampling and Hamiltonian Monte Carlo methods. In the latter case we introduce a new parameterisation of the posterior that is extremely efficient in the low signal-to-noise regime and can be readily applied to a wide range of scientific problems. We apply this methodology to a series of simulations, and to between seven and nine yr of observations for PSRs J1713$+$0747, J1744$-$1134, and J1909$-$3744 with frequency coverage that spans 700-3600MHz. We use a smooth model for profile evolution across the full frequency range, and compare smooth and piecewise models for the temporal variations in DM. We find the profile domain framework consistently results in improved timing precision compared to the standard analysis paradigm by as much as 40% for timing parameters. Incorporating smoothness in the DM variations into the model further improves timing precision by as much as 30%. For PSR J1713+0747 we also detect pulse shape variation uncorrelated between epochs, which we attribute to variation intrinsic to the pulsar at a level consistent with previously published analyses. Not accounting for this shape variation biases the measured arrival times at the level of $\sim$30ns, the same order of magnitude as the expected shift due to gravitational-waves in the pulsar timing band.

==> RefResponse <==

Many Thanks to the referee for their detailed comments.  I have marked changes in the manuscript in blue, and below I reply to the comments individually. 


p. 1 Abstract line 42. paper says improved precision 100% for DM parameters comparing profile-domain and traditional TOAs. Is this in the text of the manuscript? Figure 1 caption says the improvement is 40%. 

Response: This was left behind from a previous version, I have updated the abstract.

p. 1 Abstract line 46; (also p. 19 left col line 50). paper reports ~30 ns arrival times in J1713+0747 due to shape changes. This is not a new measurement. Cite previous work, e.g., Arzoumanian et al 2015, Fig 2. 

Response: I have updated the abstract to say it is consistent with previously published results, and added a refernce to the main text.

p. 2 left col line 2 "assuming some fiducial timing model." "Fiducial" means "assumed as a fixed basis of comparison" (OED), i.e., reference point. Not an appropriate word to describe the folding model. 

Response: Changed it to 'best available estimate of the timing model'

p. 2 right col lines 36, 42, 49. Line 36: "model vector s". Line 42: "we will parameterise the signal." Line 49: "signal vector, s(a)=Ma". Use consistent wording, either "model" (preferred) or "signal", not both. 

Response: Updated to be model.

p. 3 left col lines 9-12. "we refer to as the high S/N (HSN) parameterisation" 
... "we consider a zero S/N scenario." At a minimum this wording is confusing. 
Easiest solution: use different name scheme instead of LSN and HSN parameterization. 

Response: Changed to be 'Model parameterisation 1' (MP1) and MP2.

p. 3 left col lines 10-34 and fig 1 left top and middle. If the data were generated using unit variance, the hyper-parameter phi (standard deviation of the noise) should be found to be close to 1, and hence rho=log10(phi) be close to zero. This is not the case in the upper and middle panels figure 1, either on the left or right side, where the probability of rho being zero is very small, and the posterior is dominated by values much less than zero. Why is this? 


Response: I think this is just a misunderstanding.  The model in this case is not being fit to the unit variance noise, as the matrix N already accounts for this, as it is the identity matrix.  The model described by the amplitudes, a, and the hyperparameter, rho, is for an additional uncorrelated signal, and so should be consistent with zero, with an upper limit somewhere around a value of 1.  I have updated the text to try and make this more clear.

p. 3 left col line 40 just after equation 4. "...where as before phi_i is the model parameter describing the standard deviation of the ith amplitude parameter." Before, there was only a single phi value (under the assumption that all points were subject to the same noise) but now there are many phi_i. Taken at face value, you are now fitting 20 parameters (ten a_i, ten phi_i) to 10 data points. p. 3 left col line 55. Rho is used here without a subscript. To which phi_i does it refer? Clarify, i.e., presumably there is only one parameter phi, not ten phi_i as introduced in the previous paragraph. 

Response: There is still only one phi, I have removed the subscript for clarity.

p. 3 left col line 56. "Log-uniform and uniform priors in rho." Do you mean log-uniform and uniform in phi, as in the earlier analysis (p. 3 left col line 21)? 

Response: Yes, I have corrected this.

p. 3 right col lines 7-13. "a second high S/N toy problem in which our data vector has an additional uncorrelated stochastic component with a standard deviation of 10." (i) Add commas so this begins "a second, high S/N, toy problem...." (It isn't the "second high S/N problem.") (ii) To what is the "additional" uncorrelated component added? The figure caption says the amplitudes are ~10 sigma, but this should be in the text itself, and written more clearly. Does the amplitude of ~10 sigma, with each component having noise of 10, mean each signal is ~100? Also, why does a_1 in the lower left panel have values of -20 to -18? And why does the re-parameterisation induce a correlation between u_1 and rho? 

Response: As before I think this is a slight misunderstanding.  The 10 sigma refers to the ratio of the model amplitudes (a) to the unit variance noise.  In this toy problem each amplitude parameter is therefore in the range [ -30 → 30 ].  The reason they become correlated can be understand by considering the two parts of the likelihood.  There is the 'data part' (d – Ma), and the 'prior part' (a^T phi^-1 a).   In the low signal to noise example, only the prior part contributes, which for the new parameterisation is independent of the value of rho (its just u^T u), but in the high signal to noise regime the data part contributes, so the signal = M * sqrt(phi) * u, which directly correlates phi and u.  I havnt added anything on that last point to the text, but let me know if you think it would be worth while.

p. 3 right col line 42 and later "scale factor Lambda". Is Lambda a fixed parameter for a given pulsar, or is it fit along with other model parameters? If it is fixed, how is it determined? If it is not fixed, how is interpolation (section 3.2) done, as the interpolated model would depend on Lambda as well as profile rotation? (I later found these matters to be addressed on page 6, section 3.4. At a minimum, p. 3 should say that this will be discussed in section 3.4.) 

Response: Ive mentioned this in the interpolation section.

p. 3 right col line 49 equations 7 and 8. The basis functions B_n are not orthonormal. They would be orthonormal if the exponential factor in equation 8 were Exp(-t^2/4) rather than Exp(-t^2/2). Is this a typo? If not, why choose non-orthogonal basis functions? 

Response: There was a typo.  I have corrected this equation.


p. 4 fig 1. Add x-axis labels to the a_1 and u_1 one-dimensional plots (for readers unfamiliar with triangle plots). 

Response: Done

p. 5 left col line 4 in "amplitude ... which we then scale in amplitude for each epoch" and line 11 "overall scaling factor for a particular epoch": the amplitude scale depends on frequency as well as epoch (due to scintillation). 

Response: Updated to say that the amplitude parameter is for every profile in the data set, not just every epoch.

p. 5 left col line 20 equation 11 and text immediately preceding it. B_m is written as a function of t+\delta\phi, but "t" implies time units (e.g. seconds) whereas "\delta\phi" implies phase units (e.g. radians). 

Response: I've now stated that delta phi is in units of time.

p. 5 right col line 26 "N_i,j values representing the amplitude of the profile". Previously (e.g., equation 10), "amplitude" meant an overall scaling factor, but here it means flux density at a given pulsar phase. Change "amplitude" to "flux density" here, or find some other way to distinguish these quantities. 

Response: Changed to flux density

p. 5 right col line 32, "arbitrary baseline offset gamma_i,j." Why is arbitrary amplitude A incorporated into the parameters collectively called theta (p. 5 left col line 27), but arbitrary baseline gamma is not? Better to explicitly include A_i,j in equation 12, s_i,j(...A_i,j,gamma_i,j) = A_i,j s(...)+gamma_i,j. 

Response: I have added gamma into Eq. 10, and propogated this onwards.

p. 5 right col line 56 (continuing on p 6) "a global scaling factor, referred to as EFAC". (i) Is this used for both the GHS and Polychord analyses? (ii) Traditionally (e.g. tempo2), EFAC refers to scaling of time domain errors, not rms baseline errors as used here. In principle they should have the same effect, but it would be good to point out the difference in EFAC definitions in the manuscript. 

Response: The EFAC parameter isn't included in the GHS analysis, as the rms baseline error in the profile is a free parameter for every profile.  I've restructured this paragraph to make this more clear, and referred to the TOA case.

p. 6 left col line 30 equation 14. zeta_i,k on the right hand side should not depend on nu. 

Response: Corrected

p. 6 left col line 37 equation 15. For consistency with earlier notation, s and B_n should be functions of t, not x. 

Response: Corrected 

p. 6 left col lines 37-42. equations 15, 16. Confusing that Lambda refers to both Lambda(nu,lambda) (RHS of equation 15 and LHS of equation 16) and the specific value of Lambda at nu=nu_c (LHS of equation 15 and RHS of equation 16). Change Lambda to Lambda_0 or similar notation in LHS of equation 15 and RHS of equation 16.

Response: Updated to Lambda_c for clarity. 

p. 6 left col line 56 equation 19. lambda (lower case) as used in equations 16 and 19 is inconsistent, e.g., it has dimension 1/frequency in equation 16 but is dimensionless in equation 19 (since w has same units as s). I have been unable to check these equations as a result. Also, equation 19 appears to be a linear expansion about a fiducial value of Lambda (the value at nu=nu_c, which I suggested calling Lambda_0) but there is no explicit dependence on this in the equation as written. 

Response: I've added in the Lambda_c explicitly.  Eq 19 was missing a factor of (nu – nu_c), so they should now be consistent.

p. 6 right col lines 20-24 equations 20-21. A single equation is given two equation numbers (20 and 21). 

Response: Fixed

p. 6 right col lines 20-27 equations 20-22. I have not been able to reproduce equation 20/21. For time derivatives of B_n, Mathematica gives expressions dependent on H_(n-1) and H_n rather than H_(n-1) and H_(n+1) as in the manuscript. I have not attempted to apply Hermite polynomial recursion relations to this problem. Could the authors provide a derivation of equation 20/21? It should not go into the paper itself, but I would like to verity it. The same applies for equation 17; it would be easiest if the authors provided their derivation. 

Response: The derivation is attached as a separate file.  It uses two equations relating the derivatives of the hermite polynomials to higher and lower order terms.  Those can be verified in Mathematica.  There was a missing factor of 1/Lambda_c in Eq 17 which has been added.  The error in the Eq for the shapelet model would also have contributed to some confusion I imagine.

p. 6 right col line 44. "hyper-parameter J_i is the theoretical standard deviation of the jitter model". (i) What is meant by "theoretical"? There is no known theory of jitter. (ii) Change "standard deviation of the jitter model" to a more meaningful phrase such as "standard deviation of arrival time shifts due to jitter." 

Response: Updated to '..is the standard deviation of the arrival time shifts due to the jitter model..”

p. 7 left col line 26 "W represents the theoretical standard deviation...." Again what is meant by "theoretical"? 

Response: Similarily updated.

p. 7 left col line 35 "scale of the fluctuation in phase space." Change "phase space" to "pulse phase" or some other term. "Phase space" has a general meaning in classical mechanics that has different connotations than is meant here. 

Response: Updated

p. 7 section 3.7 in general. "High-frequency" and "low-frequency" are misnomers. The stochasticity model in section 3.7.1 is based on time domain functions (different variance in each bin). The stochasticity model in section 3.7.2 is based on frequency domain functions (shapelets). Either "high-frequency" or "low-frequency" noise would potentially affect all bins in the analysis in 3.7.1, and would potentially only affect some subset of shapelets in section 3.7.2. There is nothing intrinsically "high-frequency" about 3.7.1 or "low-frequency" about 3.7.2. 

Response: I've changed this to uncorrelated in phase, and phase-correlated noise.  Hopefully that is more clear?

p. 7 left col lines 45-50 (i) "proportional to the mean profile" (line 48) is confusing, because it can be mis-read as the mean profile amplitude. (ii) "constant increase" (line 49) is confusing: what is increasing? Fix these by changing "we will consider a two component model for the stochastic envelope" to "we model the stochastic envelope as the sum of two terms" (line 46), by changing "proportional to the mean profile" to "proportional to the profile" (line 48), and by changing "a constant increase" to "a constant in increase in the uncorrelated noise across..." to "a second term that is constant across...." (line 49). Also, "peak amplitude" should simply be "amplitude" (line 50), given the definition of A_i,j. 

Response: Updated

p. 7 left col line 56. delta_01. This is strange notation, it looks like a Kronecker delta function that always has value 0 since the indexes 0 and 1 are never equal. 

Response: Changed to delta_p

p. 7 right col lines 5-15. Paragraph "When sampling ... in Eq (27)." This paragraph is confusing. (i) "In order to scale alpha and beta for each profile." If they are "being scaled" what are they being scaled relative to? (ii) Fd is the flux in the on-pulse region, F_m is the flux of the mean profile. Aren't these the same thing, since the "on-pulse" region is where all the flux is (by definition of on-pulse)? And aren't alpha and beta global parameters in the fit (hence there is no need to re-scale them)? Clarify this. 

Response: I've updated this to be more clear.  Fd is the flux in the data, whereas F_m is the flux in the model, with A=1.  This means F_d/F_m is the maximum likelihood amplitude for the profile model.  This is needed in eq 26, as alpha and beta are defined relative to the amplitude of the profile in a particular epoch.

p. 7 right col line 36 equation 29. The variable "i" has two different meanings in this equation, (i) ith shapelet coefficient (ii) epoch i. Fix this. 

Response: Fixed, the epoch is now k.

p. 7 right col line 40 "P_d,i is the power in the on pulse region." Does "power" mean the same thing as "flux" (e.g., near equation 28) or "amplitude" (elsewhere in the paper)? If so, use consistent wording. If not, clarify what it means. 

Response: Updated to make clear that power means F_d^2.

p. 8 left col line 6. Define N_m in this paragraph, near its first use. Don't wait until the next paragraph to define it. 

Response: Done.

p. 8 left col line 13 after "for each channel j" add "and phase bin k". (Presently k is not defined.) 

Response: Added.

p. 8 left col line 26. N_i is not defined. You can get away with this by starting that sentence "Adopting the notation of that paper, we define...." 
.
Response: Done.

p. 8 left col line 28 "probability distribution for the remaining non-linear parameters." What does "remaining" mean here? Clarify. 

Response: I took out the word 'remaining', it is simple all the non linear parameters.

p. 8 right col line 47. "tempo2." Give a reference URL or paper. 

Response: Added footnote with URL.

p. 8 right col 55. "change in the ToAs can be described completely by a yearly term ... higher frequency terms that arise...." This implies that tempo2 only incorporates an annual sinusoid in this calculation, but its actual algorithm is more accurate than that; it fully incorporates the position and velocity of the observatory relative to the SSB. The tempo2 algorithm assumes small variations in astrometry parameters and hence linear changes, but this is reasonable. It does not incorporate relativistic propagation. Is this the issue you are addressing? Clarify. 

Response: I've updated this.  I couldn't reproduce the issue I had initially with the most recent version of the code, and I agree that higher order terms shouldn't affect the linear approximation when sampling the small variations about the best fit.

p. 9 left col line 20 equation 33. bold-face j_j is not explicitly defined, but the text hints that it is a matrix of jitter profiles as in equation 20. However, equation 33 is "data minus jitter". Shouldn't it be "data minus model-of-standard-profile- 

Response: It should have both, I have corrected the equation.

p. 9 left col line 41 "assuming 256 MHz of bandwidth". Give the number of channels here (32 channels of 8 MHz bandwidth) instead of giving it two paragraphs later. 

Response: Done

p. 9 right col lines 31-32 and p. 10 fig 3. Units of microseconds are used in the text for EQUAD and uncertainty, but units of seconds are used in the figure. Use consistent units. 

Response: Changed to be seconds in the text.

p. 9 right col line 41. "only the first [FD] term is required." Given the dramatic change in profile across the band, this is surprising. How did you determine that only the first term is required? (Specify this in the manuscript.) 

Response: Looking at the covariances with tempo2 -output matrix, FD1 and FD2 are almost 100% correlated, I imagine due to the narrow bandwidth.  We simply tried adding higher order terms into the par file, and found that they were all consistent with zero.

p. 9 right col line 44. "no evidence of additional scatter in this data set." Clarify, what do you mean "additional scatter" ("additional" to what)? And which data set does this apply to -- you discuss many analyses of multiple data sets in the previous paragraph and in this paragraph, it isn't clear which you are referring to at this point. 

Response: I have rephrased this to say no evidence of an equad when using the 8MHz ToAs and including FD1.  

p. 9 right col line 52 "FD parameters are more covariant with the timing model parameters than the [shapelet amplitude] parameters that describe profile evolution." This is surprising. Both FD and and shapelet-amplitude parameters describe pulse evolution over frequency, and both are constant in time, so both should be close to orthogonal to frequency-independent, time-dependent timing parameters (i.e., everything except DM). 

Response: I've changed the discussion quite a bit here.  I agree that the FD parameter should not be signficantly correlated with other timing parameters.  The improvement comes because the error bars on the ToAs have a frequency dependent scaling (figure included in the paper), due to the profile evolution and the template mismatch that this causes.  The EFAC/EQUAD parameters cannot model this correctly, and so this causes the overall decrease in sensitivity compared to the profile domain analysis.

p. 10 Figure 3. The panels in this figure are largely independent of each other. Consider splitting it into multiple figures. 

Response: While I agree they are somewhat independent, I find it slightly tidier if they're all together.

p. 10 right col line 52. Define what is meant by "DMX parameterization" and describe the time scale used for DMX in your simulations (looks like separate DMX at each epoch?). 

Response: I have now described it as a piecewise-constant DM(t) model, which is specified for each epoch in the data set.

p. 11 Table 2. Explicitly define "F-averaged" (in the text or in a footnote). 

Response: Ive simply called it 'Frequency Averaged' as there was space in the table.

p. 12 left col section 5. State whether both the 10/40 and the 20 cm receivers are used at every epoch, and if the observations are close together in time. 
p. 18 left col line 38. "J1909-3744 ... binary period is ~1.5 days ... shorter than the 30-day window used in the DMX model." Your observing interval is stated to be 3 weeks, in which case most 30-day DMX windows have only one observation, i.e, they will be measured over a very short period of time. 

Response: The three week statement has been corrected, the mean difference between observations is 2 weeks, with a standard deviation of 10 days for each of the three systems used.  In total the mean separation is 6 days, so while the 10/50 are simultaneous, the 20cm is typically offset by a few days. Thus there are multiple observations in each DMX window.

p. 12 left col line 54. "A firmware upgrade for the DFB systems allowed the signals to be referenced to the digitiser, resulting in a jump...." This is incomprehensible to someone not familiar with your hardware. (Why would referencing signals to the digitiser cause an arbitrary offset?). Best to reduce the level of detail. 

Response: Removed most of the detail, simply said jump was the result of a firmware upgrade.

p. 12 right col line 28. "(IPJ) Interpulse jitter." Clarify that this means the model in which two components are allowed to have separate jitter parameters. Or else explicitly define the term "interpulse jitter" at the end of section 3.5, where the mathematical description of this model is given. 

Response: Now defined at the end of section 3.5.

p. 12 right col line 46. In the fractional changes in profile widths, what is the significance of the sign (define it in the text)? 1713 is positive, the other two negative; from fig 6, all three pulsars have decreasing width with increasing frequency. Does this pattern reverse for 1713 within the 10 cm band? 

Response: Stated that negative values reflect a decrease in width with increasing frequency.  For the main peak in the profile for 1713 It does narrow, however the evolution of the profile as a whole is quite complex, and so a single nuber denoting a change in width is somewhat meaningless in that case.  I've made a statement to this effect in the text.

p. 14 right col line 42. "neighboring channels are still consistent to within 2 sigma." What exactly does this mean: that all bins are consistent within 2 sigma where sigma is defined by noise? Or they are indistinguishable with 95% confidence ("2 sigma") according to some statistical measure (what measure)? Or something else? 

Response: It meant that the maximum difference between the models at any point in phase between neighbouring channels is less than 2 sigma.  I've updated the text to clarify.

p. 14 figure 7 caption. "curvature is a result of the uncertainty in the model for profile evolution gradually dominating over the uncertainty in the mean profile." Not obvious how this works. Clarify. 

Response: The uncertainty in the mean profile at any frequency is a constant, whereas the uncertainty in the model for profile evolution grows as the frequency difference grows.  i.e., for a linear model the error increases linearly as delta in frequency increases.  I've updated the caption.

p. 14 right col line 45. after "magnitude of the profile evolution being much greater in the PSR J1744-1134 data set", add "while the timing uncertainty of PSR J1909-3744 is much smaller," or reword the sentence in some other way to clarify this point. 

Response: Updated

p. 15 Table 4. For the IPJ model, does your model assume the two separately modeled components (main pulse and interpulse) have the same jitter parameter? Clarify this in the text. (If they have separate jitter parameters, then report both of the parameters for J1744-1134, though the text hints (p. 16 left col line 37) that the interpulse jitter is largely unconstrained). 

Response: For the IPJ model the model fits for the variation in delta phi (the seperation in phase between the two components).  I've restated this in the text at this point.

p. 15 right col line 23. "...J1713+0747 ... correctly modelling such shape variation will become more important as the sensitivity of observations improves by even a factor of a few." Future tense ("will become") is inaccurate. This is already an issue in larger EPTA and NANOGrav telescopes. You could cite, e.g., Demorest et al 2013 or Arzoumanian et al 2015. 

Response: Added something to this effect, referencing the recent EPTA/PPTA/NG papers.

p. 16 right col line 47. "include periods in our model from 1/T...." 1/T is a frequency, not a period. 

Response: Correct.

p. 16 right col line 49 "non-stationary DM event ... J1713+0747" give a reference for this event. 

Response: Added

p. 18 Figure 11. J1909 is shown has having a low spectral index, but the DM vs time plot in figure 10 has a very large long-term trend, i.e., it is dominated by the longest time scales and hence very red. Your choice of removing a quadratic in DM severely distorts the DM spectrum analysis of this source. 

Response: The analysis doesn't 'remove' the quadratic though. The quadratic is fit simultaneously with the power law model, which therefore essentially fits for the non-smooth part.  One could also argue that the linear part isn't stochastic in nature, and so including that as part of the model for the turbulent stochastic signal would skew the result the other way.

p. 18 right col line 53. Decrease in timing precision of J1713+0747. Quantitative analysis of this (~30 ms) is only given in section 7 (conclusions); it would be more better to include it in section 6.5 (timing precision) as well. (Also, see my comment about this effect in my comments about the paper abstract, above.) 

Response: A discussion of the impact of this is given in section 6.2.1, unless I misunderstand the part of the text you are referring to.

p. 19 left col line 15 for "time of arrivals" write "times of arrival." Also line 43. 

Response: Changed

p. 19 left col line 34. "additional five years ... for a nine year data set"; but page 18 gives this same result using time spans of four and seven years. Both are correct, but pick one or the other and use it consistently to avoid confusing the reader. 

Response: Changed to four/seven.

p. 19 left col line 43 "Recently introduced methods for simultaneously estimating the DM with the pulse time or arrivals will be unable to leverage this additional constraint [smoothed DM variations]." Incorrect. Traditional timing models (chi^2 minimization in frequentest framework) minimize differences between measured times and model times, but the chi^2 calculation can be extended to also include difference between measured DM (at every epoch) and model DM. This capability exists in tempo1. 

Response: I have removed the statement.

References. For arXiv references, the arxiv paper number is not given. 

Response: Done

Table 5. Give epochs of period and proper motion. 

Response: Done

Table 5, Section 6 or 7. Please compare the timing parameters in table 5 with previous work (e.g. Reardon et al 2016 or similar papers from EPTA or NANOGrav), both in terms of uncertainties and in absolute values of the pulse parameters. Are there quantities for which your new analysis measures significantly different (many sigma) values than the previous analysis? This would be indicative of systematics in either the present work or (much more likely) in the older analysis. This could provide another compelling reason that profile domain timing may be superior to traditional timing.
The only significant addition I recommend is an analysis of the parameter values (not just the uncertainties) from this paper's timing of three millisecond pulsars (i.e., table 5) using the profile-domain technique. These values should be compared to the values attained via traditional timing, both by the authors themselves (they have already done the analysis but not reported the numerical results of parameter values) and by others (e.g., Reardon et al 2016). Does the profile domain analysis give systematic differences in parameter values compared to traditional analysis? Does it improve accuracy as well as formally calculated uncertainties? 

Response: I've included one extra panel in the last figure which shows the difference between the ToA and profile domain estimates from the analysis I performed. 

I’ve also added in a comparison of some of the key astrometric parameters (parallax and PM) and the binary parameters with recent publications (Desvignes 2016, Reardon 2016, Matthews 2016, Fonseca 2016).  

